A BERT-based Distractor Generation Scheme with Multi-tasking and Negative Answer Training Strategies

In this paper, we investigate the following two limitations for the existing distractor generation (DG) methods. First, the quality of the existing DG methods are still far from practical use. There is still room for DG quality improvement. Second, the existing DG designs are mainly for single distractor generation. However, for practical MCQ preparation, multiple distractors are desired. Aiming at these goals, in this paper, we present a new distractor generation scheme with multi-tasking and negative answer training strategies for effectively generating \textit{multiple} distractors. The experimental results show that (1) our model advances the state-of-the-art result from 28.65 to 39.81 (BLEU 1 score) and (2) the generated multiple distractors are diverse and show strong distracting power for multiple choice question.

==> 2.1.backup_method.tex <==
\section{BERT Distractor Generation}\label{sec:BDG}

\subsection{BERT Model Review}
The BERT model and its family \cite{liu2019roberta,lan2019albert} are composed of a stack of multi-layer bidirectional Transformer encoders. The input to a BERT model is a sequence of tokens. For a given token, its input representation to BERT model is first constructed by summing the corresponding token, segment, and position embeddings. After the input representation, the input embeddings travel through the pre-trained/fine-tuned BERT for task learning and prediction. In general, BERT can be employed in two-level language modeling tasks: sequence-level classification and token-level prediction tasks. For the tasks, there are three special tokens, \texttt{[C]}, \texttt{[S]}, and \texttt{[M]}. The embedding of the \texttt{[C]} token is designed to be used as the aggregate sequence representation for classification tasks. The \texttt{[S]} is designed to distinguish different sentences of a token sequence (to provide/signal information from multiple sentences, as the input token sequence can be a pack of multiple sentences). On the other hand, the \texttt{[M]} token is designed to be used in token-level prediction (e.g., predicting a masked token based on context words or predicting the starting/ending probabilities for span-based tasks such as QA tasks).


As reported in \cite{chan2019recurrent, dong2019unified}, BERT essentially is an auto-encoder language modeling design, which aims to reconstruct the original data from corrupted inputs. If BERT is asked to predict a sequence of consecutive masked tokens, it often produces incoherent and ramble results. For example, when using BERT to predict three consecutive $\mathrm{\texttt{[M]}}\mathrm{\texttt{[M]}}\mathrm{\texttt{[M]}}$ masked tokens, the same prediction result for the tokens are often observed. This is because the context (the information for predicting the tokens) for the masked tokens are nearly the same except for the position embedding, making the generated sentences incoherent. Thus, we take into consideration the previous decoded results for decoding the next distractor token, as will be introduced in the next subsection. 


\begin{table*}
\centering
\begin{tabular}{|l|l|l|}
\hline
Iter. & Input Sequence & Predict \\ \hline
1 & \texttt{[C] $C$ [S] [M]} & they  \\ \hline
2 & \texttt{[C] $C$ [S]} they  \texttt{[M]} & don't \\ \hline
3 & \texttt{[C] $C$ [S]} they don't \texttt{[M]} & know \\ \hline
4 & \texttt{[C] $C$ [S]} they don't know \texttt{[M]} & how \\ \hline
5 & \texttt{[C] $C$ [S]} they don't know how \texttt{[M]} & to \\ \hline
5 & \texttt{[C] $C$ [S]} they don't know how to  \texttt{[M]} & get \\ \hline
6 & \texttt{[C] $C$ [S]} they don't know how to get  \texttt{[M]} & out \\ \hline
7 & \texttt{[C] $C$ [S]} they don't know how to get out  \texttt{[M]} & of \\ \hline
7 & \texttt{[C] $C$ [S]} they don't know how to get out of \texttt{[M]} & the \\ \hline
7 & \texttt{[C] $C$ [S]} they don't know how to get out of the \texttt{[M]} & building \\ \hline
8 & \texttt{[C] $C$ [S]} they don't know how to get out of the building\texttt{[M]} & \texttt{[}S{]} \\ \hline
\end{tabular}
\caption{A Running Example for the BDG scheme}
\label{tab:dg}
\end{table*}

% \begin{table*}
% \centering
% \begin{tabular}{|l|l|l|}
% \hline
% Iter. & Input Sequence & Predict \\ \hline
% 1 & \texttt{[C] $C$ [S] [M]} & We \\ \hline
% 2 & \texttt{[C] $C$ [S]} We \texttt{[M]} & should \\ \hline
% 3 & \texttt{\begin{tabular}[c]{@{}l@{}}{[}C{]} $C$ {[}S{]} We should {[}M{]}\end{tabular}} & avoid \\ \hline
% 4 & \texttt{\begin{tabular}[c]{@{}l@{}}{[}C{]} $C$ {[}S{]} We should avoid {[}M{]}\end{tabular}} & air \\ \hline
% 5 & \texttt{\begin{tabular}[c]{@{}l@{}}{[}C{]} $C$ {[}S{]} We should avoid air {[}M{]}\end{tabular}} & pollution \\ \hline
% 6 & \texttt{\begin{tabular}[c]{@{}l@{}}{[}C{]} $C$ {[}S{]} We should avoid air pollution.{[}M{]}\end{tabular}} & \texttt{[}S{]} \\ \hline
% \end{tabular}
% \caption{A Running Example for the BDG scheme}
% \label{tab:dg}
% \end{table*}

\subsection{BERT-based Distractor Generation (BDG)}\label{sec:BDG_architecture}


In a distractor generation scenario, there are three given inputs: (1) a paragraph $P$, (2) an answer $A$, and (3) a question $Q$. For ease of discussion, let $C$ (referred to as a context sequence) denote the sequence of tokens given by concatenating $P$, $Q$, and $A$. 

Our BDG model generates distractor tokens in an auto-regressive manner. Specifically, the BDG model predicts a token at a time based on (1) the given context sequence $C$ and (2) the previously predicted distractor tokens. The BDG model takes multiple iterations to generate a distractor. In Table \ref{tab:dg}, we show a running example for the BDG model. Note that at each iteration, our model predicts a token based on $C$ and the previous generated tokens. For example, at Iteration 1, we generate "they" based on $C$. At Iteration 2, we generate "don’t" based on $C$ and "they" tokens, and Iteration 3, we generate "know4" based on $C$, "they", and "don’t". The generation terminates when \texttt{[S]} is predicted. In this example, "they don’t know how to get out of the building" is the final generated result. 

Specifically, the input sequence $X_{i}$ at Iteration $i$ to BERT is 
\[ \begin{split}
X_{i} = (\mathrm{\texttt{[C]}}, C, \mathrm{\texttt{[S]}},\hat{d_{1}}, ...,\hat{d_{i}},\mathrm{\texttt{[M]}})
\end{split} \]
Let $\mathbf{h}_{\texttt{[M]}} \in \mathbb{R}^h$ denote the hidden representation of \texttt{[M]} of $X_{i}$ returned by BERT transformer stacks. The prediction of $\hat{d_i}$ is given by a linear layer transformation $\mathbf{W}_{\texttt{DG}} \in \mathbb{R}^{h\times |V|}$ and a softmax activation to all vocabulary dimension as follows.  
$$p(w|X_i) = softmax(\mathbf{h}_{\texttt{[M]}}\cdot\mathbf{W}_{\texttt{DG}}+\mathbf{b}_{\texttt{DG}})$$ 
$$\hat{d_{i+1}}= \mathrm{argmax}_w {Pr(w|X_i)} $$

% For a given paragraph $P$ = [$p_1, ..., p_{|C|}$], an answer $A$ = [$a_1, ..., a_{|A|}$], and a question $Q$ = [$q_1, ..., q_{|Q|}$], our BDG (BERT Distractor Generator) scheme generates distractor tokens based on (1) the given context (i.e., $P, A, Q$) and (2) the previously predicted distractor tokens. 

% Let $C$ denote $P\oplus Q\oplus A$, the sequence of context tokens () for distractor generation. With $C$, the input sequence $X_{i}$ to BERT is 
% \[ \begin{split}
% X_{i} = (\mathrm{\texttt{[C]}}, C, \mathrm{\texttt{[S]}},\hat{d_{1}}, ...,\hat{d_{i-1}},\mathrm{\texttt{[M]}})
% \end{split} \]
% Let $\mathbf{h}_{\texttt{[M]}} \in \mathbb{R}^h$ denote the hidden representation of \texttt{[M]} of $X_{i}$ returned by BERT transformer stacks. The prediction of $\hat{d_i}$ is given by a linear layer transformation $\mathbf{W}_{\texttt{DG}} \in \mathbb{R}^{h\times |V|}$ and a softmax activation to all vocabulary dimension as follows.  
% $$p(w|X_i) = softmax(\mathbf{h}_{\texttt{[M]}}\cdot\mathbf{W}_{\texttt{DG}}+\mathbf{b}_{\texttt{DG}})$$ 
% $$\hat{d_{i+1}}= \mathrm{argmax}_w {Pr(w|X_i)} $$

Subsequently, the newly generated token $\hat{d_i}$ is appended into $X_{i+1}$ and the distractor generation process is repeated based on the new $X_{i+1}$ until \texttt{[S]} is predicted. Our loss function is as follows.
$$\underset{\theta}{\text{minimize}}-\sum_{\forall (C,  D)} \sum_{i=1}^{|D|}(\text{log}_2p(d_{i+1}|{C, d_{1:i};\theta}))$$



% An Example for our BDG model: Passage $P$: Chocolate is good for your heart ... (see Appendix\ref{app:BDG example} for the full context paragraph), Question $Q$ : What is the best title for this passage?, Answer $A$: Chocolate, a Healthy Food. 
% \subsection{Sequential Masked Language Model}\label{sec:SMLM}
 
\subsection{Answer Negative Regularization}
From the experiment results (will be presented in the later section), we see the BDG model advances the state-of-the-art result \cite{zhou2019coattention} from 28.65 to 35.30 (BLEU 1 score). While the token-level evaluation result looks promising, we find that generation results still have room to be improved. One observation is that in many cases, there is an \textit{answer copying problem} for generating distractors; the generated distractors are similar to the given answers. To better see this phenomenon, we conduct an experiment to count such cases. In the following table, we show the number of cases that the generated distractor $\hat{D}$ has a token-level similarity score greater than $0.95$ with respect to the answer $A$. We also show the cases for the gold distractors. By comparison, there is a significant gap between the human invented distractors and the model generated ones. 
\\\\
\begin{tabular}{|l|l|l|}
\hline
 & BDG & Gold \\ 
\hline
\# of cases on BLEU1   & 115 & 12 \\ \hline
\# of cases on BLEU2   & 115 & 4 \\ \hline
\# of cases on BLEU3   & 109 & 0 \\ \hline
\# of cases on BLEU4   & 97 & 0 \\ \hline
\# of cases on ROUGE-L   & 122 & 1 \\\hline
\end{tabular}
\\\\

Motivated by the answer copying problem, we propose to incorporate a loss (referred to as \textit{answer negative loss}) to discourage predicting tokens in $A$ when predicting $\hat{d_i}$. With the answer negative loss, our loss function for BDG is as follows.

\begin{equation}
\begin{split}
&\underset{\theta}{\text{Minimize}}-\sum_{\forall (C, D)}\phi_{_{a.n.}}(C,D), \\
& \begin{split}
    \phi_{_{a.n.}}=&\sum_{i=1}^{|D|}(\text{log}_2p(d_{i+1}|{C,d_{1:i};\theta})+\\&\sum_{\forall a_j\in A}\text{log}_2(1-p(a_{j}|{C;\theta}))  
    \end{split}
\end{split}
  \label{eq:SLUL}
\end{equation}

% Note that $\beta$ is a hyper-parameter controlling the weighting of answer negative loss. We conduct experiments to observe the effect of the $\beta$ value (See Subsection \ref{subsec:parameter_study}).

% The design of answer negative loss is motivated by the observation that compared with the entire context article, we found that answer and distractor are relative short phrases. By statistics, the averaged article length of RACE data set is 274 tokens, and distractor, question and answer phrases are 8.3 tokens in average. Under such a circumstance, the model 


% \begin{equation}\small\begin{split}
%   \underset{\theta}{\text{minimize}}-\sum_{\forall (C, D)}& \sum_{i=0}^{|D|}(\text{log}_2p(d_{i+1}|{C, d_{1:i};\theta}))\\ &+\sum_{j=1}^{|A|}\text{log}_2(p(d_{j}|{C, ;\theta}))
%   \end{split}
%   \label{eq:SLPL}
% \end{equation}

% \begin{equation}\small\begin{split}
%   \underset{\theta}{\text{minimize}}-\sum_{\forall (C, D)}& \sum_{i=0}^{|D|}(\text{log}_2p(d_{i+1}|{C, A, d_{1:i};\theta})\\ 
%   &+\sum_{j=1}^{|A|}{log}_2(1-p(a_{j}|{C, A, d_{1:i};\theta})\\  &+\sum_{j=1}^{|A|}\text{log}_2(1-p(a_{j}|{C, A;\theta})))\end{split}
%   \label{eq:SLUL}
% \end{equation}

The design of answer negative loss is motivated by the the desiderata that we expect to regulate the generated distractor $\hat{D}$ to use words different from $A$.

\subsection{Multi-task with Parallel MLM}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.88\columnwidth]{Multi-tasking.png}
    \caption{The Multi-tasking Architecture}
    \label{fig:Multi_task}
\end{figure}

In addition to the answer negative loss, we further propose to jointly train BDG and a parallel MLM (P-MLM) architecture for distractor generation to enhance the quality of BDG. The P-MLM scheme for generating distractors is structured as follows. 

For a given context $C$, the input sequence $X$ to P-MLM model is formulated as
\[ \begin{split}
X = (\mathrm{\texttt{[C]}}, C, \mathrm{\texttt{[S]}}, \mathrm{[\texttt{M}]_{d_0}}, \mathrm{[\texttt{M}]_{d_1}}, ...,\mathrm{[\texttt{M}]_{d_{|D|-1}}})
\end{split} \]
Let $\mathbf{h}_{\mathrm{\texttt{[M]}_{d_i}}} \in \mathbb{R}^h$ denote the hidden representation of $\mathrm{\texttt{[M]}_{d_i}}$ of $X$ returned by BERT transformer stacks. The prediction of $\hat{q_i}$ is given by a linear layer transformation $\mathbf{W}_{\texttt{P-MLM}} \in \mathbb{R}^{h\times |V|}$ and applying a softmax activation to all vocabulary dimension as follows.  
$$p(w|X) = softmax(\mathbf{h}_{\mathrm{[\texttt{M}]_{d_i}}}\cdot\mathbf{W}_{\texttt{P-MLM}}+\mathbf{b}_{\texttt{P-MLM}})$$ 
$$\hat{d_{i}}= \mathrm{argmax}_w {Pr(w|X)} $$
The loss function for P-MLM is 
$$\underset{\theta}{\text{minimize}}-\sum_{\forall (C,  D)}\phi_{_{\texttt{P-MLM}}}(C,D)$$
$$\phi_{_{\texttt{P-MLM}}}(C,D)=\sum_{\forall d_i}\text{log}_2p(d_i|{C, \mathrm{[\texttt{M}]_{d_j}};\theta})$$


We propose to jointly train P-MLM and BDG by the following multi-tasking loss function. Note that $\gamma$ is a hyper-parameter controlling the weighting of answer negative loss. See also the effect of the $\gamma$ value in Subsection \ref{subsec:parameter_study}. 
\begin{equation}
\underset{\theta}{\text{Minimize}}-\sum_{\forall (C, D)}[\phi_{_{a.n.}}(C,D)+\gamma\cdot\phi_{_{\texttt{P-MLM}}}(C,D)]
  \label{eq:SLPL}
\end{equation}



The multi-task design is motivated by the following observations. First, as mentioned, we target at learning distractor generation from real reading comprehension examination (RACE-like MCQ), and we find that many questions in the RACE dataset are summary-oriented or making inferences about a certain detail in the article; That is, many questions ask like "what is the best title for this passage?" or "what is this passage about?" Such questions require the model to have capability of passage semantic summarization. While the original BDG scheme design successfully generates fluent question sentences, we find that it may over-fit in sentence writing and under-fit in learning the passage semantic understanding capability. Note that the sequential-MLM design (BDG) essentially is a one-by-one masked token prediction architecture. Such a method may over-focus on the guess of a single token and ignore the overall semantic understanding. Thus, we propose to incorporate the multitask learning setting to prevent the potential over-fitting problem. From the experiments, we find the multi-task learning setting indeed improves the quality of distractor generation. Also, in the experiment section, we show an ablation study to examine the various parameter setting to observe the effects on the distractor generation. 

% {\color{red}
% \section{Combine AN and PM}
% We observe that our Answer Negative Regularization will cause a dropdown of token score. We guess that this is because the additional constraint result of Answer Negative Regularization cannot be the answer, making the generation of the difficulty more difficult
% Therefore, we can use Multi-task with Parallel MLM to ease the difficulty of Answer Negative Regularization, combine the two, and make the model more in the direction of generation.
% }

\section{Multiple Distractor Generation}\label{sec:MDG}
\subsection{Selecting Distractors by Entropy Maximization}\label{sec:EM}
As mentioned, another point that can be improved for DG is that the existing methods mainly focus on single distractor generation. For having more than one distractor, the existing practices is to select the results on different beam search paths as multiple options for distractor generation, which lowers the power of distracting a reader for MCQ preparation. 

Our viewpoint is that we should deal with the multiple distractor selection problem by selecting a distractor set rather than individually selecting top-k distractors based on prediction probability.

Based on this view, we propose to incorporate a multi-choice reading comprehension (MRC) model for ranking/selecting distractor sets. First, let $\mathbb{M}_{\texttt{MRC}}$ be a MRC model. Note that $\mathbb{M}_{\texttt{MRC}}$ takes a passage $P$, a question $Q$, and a set of options (including an answer phrase $A$ and distractors $D_1, D_2, ..., D_n$) as input and outputs [$p_A, p_{D_1}, ...,p_{D_n}$] as the answer probabilities of the options. $\mathbb{M}_{\texttt{MRC}}$ is trained by maximizing the answer probability $p_A$ while minimizing the probabilities [$p_{D_1}, ...,p_{D_n}$]. 

With $\mathbb{M}_{\texttt{MRC}}$, our idea is as follows. First, let $\mathbb{DG}_{\texttt{BDG}}$ be the BDG model for distractor generation. Also, let $\hat{D}=\{\hat{d}_1, \hat{d}_2, ..., \hat{d}_n\}$ be the set of generated distractors by the BDG model. In a common MCQ setting, there are four options (one answer $A$ and three distractors $d_i, d_j, d_k$) for each question. Our idea is to enumerate all possible triples from $\{\hat{d}_1, \hat{d}_2, ..., \hat{d}_n\}$. That is, we have a triple set 
\[
  \{ (d_i, d_j, d_k)| i\neq j\neq k, d_i, d_j, d_k \in \hat{D} \}
\]

For a given passage $P$, question $Q$, and answer $A$, the goal is to find a triple ($d_i, d_j, d_k$) to form an option set $O$ (i.e., \{$d_i, d_j, d_k$, $A$\} ) that maximizes the following entropy function.

\begin{equation}\label{eq:entropy}
    \underset{}{\text{maximize}}-\sum_{\forall o_i\in O}p_{o_i}log_2p_{o_i}
\end{equation}



\subsection{Model Ensemble}\label{sec:model-ensemble}
The idea of selecting distractors by entropy maximization can be further generalized by employing multiple DG models. For having multiple DG models, our idea is to leverage the variants of the BDG model (i.e., models with/without answer negative regularization or with/without P-MLM multi-task training). Let $\hat{D}, \hat{D}_{\texttt{AN}}$, and $\hat{D}_{\texttt{PM}}$ be the full DG model, the DG model without answer negative regularization, and the DG model without P-MLM multi-task training.
With the models, our goal then is to enumerate all possible triples from $\{\hat{d}_1, \hat{d}_2, ..., \hat{d}_n\}$. That is, we have a triple set as follows.
\[
  \{ (d_i, d_j, d_k)| d_i \in \hat{D}, d_j \in \hat{D}_{\texttt{AN}}, d_k \in \hat{D}_{\texttt{PM}} \}
\]

With the triple set, the options set that maximizes Eq. (\ref{eq:entropy}) is selected as final distractors.



% \noindent\textbf{RACE}
% Token level (e.g., bleu score, rouge-l) performance evaluation fail to truly reflect the quality of generated distractors. We propose to evaluate the DG quality by RACE reading comprehension task \cite{lai2017large} (Race is a large-scale reading comprehension dataset with more than 28,000 passages and nearly 100,000 questions. In the dataset, all questions contain four candidate options with only one correct option. Our idea is that a poorly generated result will reduce the difficulty of the multiple-choice task. We expect that this effect will be reflected in the phenomenon that the accuracy of a multiple choice model is improved. Thus, we propose to incorporate a RACE model to test the accuracy of a multiple choice quiz that uses the distractors generated by our model. Specifically, given $C$, $Q$, and $A$, we generate three distractors $D_1$, $D_2$, and $D_3$, and then turn the multiple choice question to the implemented RACE model. We expect that the randomly generated results will significantly increase the accuracy of the model. Therefore, we hope to reflect the quality of the results through such a way of comparison.

% In the experiment, we implement a RACE model based on  RoBERTa fine-tuned by OpenAI \cite{solaiman2019release} to realize our idea. We use the accuracy of the model as a metric. The higher the accuracy, the worse the generation quality. In Table \ref{tab:acc}, we show the results. 

% \begin{table}[ht]\centering
% \begin{tabular}{|l|r|}
% \hline
%  & \multicolumn{1}{l|}{Accuracy} \\ \hline
% Random Generator & 87.79\% \\ \hline
% Golden Distractor & 78.39\% \\ \hline
% BERT-DG & 73.39\% \\ \hline
% \end{tabular}
% \caption{Accuracy Comparison on RACE }
% \label{tab:acc}
% \end{table}





% \subsection{Generating Multiple Distractors}
% In addition to a single distractor generation, we also target at generating multiple distractors. To increase the quality of the distractors (the quality is defined in terms of increasing the difficulty of multiple-choice questions), we also employ the unlikelihood loss idea as we introduced in Eq. (\ref{eq:SLUL}) but to regulate $D_2$ use words different from the words of $A$ and $D_1$.

==> _discussion.tex <==
\subsection{Discussion}\label{sec:disc}
\subsection{Effectiveness of our a.n. and p.m. strategy}
a.n. token score seems to be lowest to others\ref{tab:one distractor token score} but in have lowest repeating score.  
a.n. can faster get to lowest evaluation loss.
\includegraphics[width=\linewidth]{loss_graph.png}     

the best setting of a.n. in loss with beta will be set as 1 \ref{tab:a.n. loss in diff setting}. 
\begin{table}
    \centering
    \begin{tabular}{|l|r|}
    \hline
     & \multicolumn{1}{l|}{Loss} \\ \hline
    a.n. beta 0.5 & 2.9975\% \\ \hline
    a.n. beta 1.0 & 2.9873\% \\ \hline
    a.n. beta 2.0 & 3.0007\% \\ \hline
    \end{tabular}
    \caption{a.n. loss in diff setting}
    \label{tab:a.n. loss in diff setting}
\end{table}

Testing in parameter, 
p.m. can give us higher token score, best setting is repeating in two times
\begin{table}
    \centering
    \begin{tabular}{|l|r|}
    \hline
     & \multicolumn{1}{l|}{BLEU 4 Token score} \\ \hline
    without p.m. & 7.16 \\ \hline
    p.m. times 1 & 7.67 \\ \hline
    p.m. times 2 & 8.95 \\ \hline
    p.m. times 3 & 8.60 \\ \hline
    \end{tabular}
    \caption{p.m. token score in diff setting}
    \label{tab:p.m. token score in diff setting}
\end{table}

\subsection{Entropy selection}
poor distractor options can make the questions almost trivial to solve
we apply our entropy selection in multi-model distractor
In this set of experimental results, we have two observations. First, the distractors generated by the random generation method are indeed not as effective as we expected. We can see that the accuracy has increased from 78\% to 88\%. Second, Although in the above experiments, we saw that the distractor produced by BDG has improved on the BLEU score compared to the existing methods. However, since the BLEU score is basically a similarity comparison based on the token level, it cannot completely represent the effect on semantic.

using beam-search with beam-size 9 to test whether we need multiple models or not.

this strategy have following benefit
- parallel inference
- better mrc score 




==> _preliminary.tex <==
\section{Preliminaries}\label{sec:preliminaries}

\subsection{Problem Formulation}
Formally, let $P$ denote the input context passage and $Q$ denote the question and $A$ the corresponding answer, respectively. The DG task is defined as generating a distractor $D$ as follows.
\begin{equation}
\hat{D} = \mathrm{argmax}_{D}\; log_2 p(D|P, Q, A)
\end{equation}

\subsection{BERT Model Review}
% Bidirectional Transformer models (i.e., BERT and its variant) are the current state-of-the-art when it comes to different NLP tasks. The BERT model is built by a stack of multi-layer bidirectional Transformer encoder \cite{vaswani2017attention}. 

The BERT model and its family \cite{liu2019roberta,lan2019albert} are composed of a stack of multi-layer bidirectional Transformer encoders. The input to a BERT model is a sequence of tokens. For a given token, its input representation to BERT model is first constructed by summing the corresponding token, segment, and position embeddings. After the input representation, the input embeddings travel through the pre-trained/fine-tuned BERT for task learning and prediction. In general, BERT can be employed in two-level language modeling tasks: sequence-level classification and token-level prediction tasks. For the tasks, there are three special tokens, \texttt{[C]}, \texttt{[S]}, and \texttt{[M]}. The embedding of the \texttt{[C]} token is designed to be used as the aggregate sequence representation for classification tasks. The \texttt{[S]} is designed to distinguish different sentences of a token sequence (to provide/signal information from multiple sentences, as the input token sequence can be a pack of multiple sentences). On the other hand, the \texttt{[M]} token is designed to be used in token-level prediction (e.g., predicting a masked token based on context words or predicting the starting/ending probabilities for span-based tasks such as QA tasks).

==> old_sec_multiple_distractor.tex <==
\section{Multiple Distractor Generation}\label{sec:MDG}
\newcommand\BDGname{BDG~}



\subsection{Selecting Distractors by Entropy Maximization}\label{sec:EM}
As mentioned, another point that can be improved for QG is that the existing methods mainly focus on single distractor generation. For having more than one distractor, the existing practices is to select the results on different beam search paths as multiple options for distractor generation.However, the distractors generated in such a manner are essentially from the same latent representation, and might have similar tokens or semantics, which lowers the power of distracting a reader for MCQ preparation. In Table \ref{tab:my-table-mdg}, we show two examples for this problems. In the illustrated examples, one can observe that the generated distractors are with the same semantics with/without similar tokens. 
% {\color{red}experiment result on token score shows that it perform much higher with beam search and mutiple-distractor training}
\begin{table}[ht]
\resizebox{\linewidth}{!}{
\begin{tabular}{l}
\textbf{Example 1} \\ \hline
\multicolumn{1}{|l|}{\textbf{Question}} \\
\multicolumn{1}{|l|}{$\cdot$ After reading the passage, we may know that} \\
\multicolumn{1}{|l|}{\textbf{Answer}} \\
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}} $\cdot$ it is better if the website domain name is related to \\ the products you sell .\end{tabular}} \\
\multicolumn{1}{|l|}{\textbf{Gen. Distractors}} \\
\multicolumn{1}{|l|}{$\cdot d_1:$ it’s easy to start your business online} \\
\multicolumn{1}{|l|}{$\cdot d_2:$ it is easy to start a business online now} \\ \hline
 \\
\textbf{Example 2} \\ \hline
\multicolumn{1}{|l|}{\textbf{Question}} \\
\multicolumn{1}{|l|}{$\cdot$ Which is Professor Jean Krutmann’ s opinion ?} \\
\multicolumn{1}{|l|}{\textbf{Answer}} \\
\multicolumn{1}{|l|}{$\cdot$We should take action to control air pollution} \\
\multicolumn{1}{|l|}{\textbf{Gen. Distractors}} \\
\multicolumn{1}{|l|}{$\cdot d_1:$ We should avoid air pollution.} \\
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}$\cdot d_2:$ We should protect our environment from dirty \\ air.\end{tabular}} \\ \hline
\end{tabular}
}
\caption{Examples for Distractors Selected by Beam Search: In these example, the distractors are with the same semantics}
\label{tab:my-table-mdg}
\end{table}


Our viewpoint is that we should deal with multiple distractor selection problems from the perspective of set, rather than individually selecting top-k distractors based on prediction probability. In other words, we should choose a distractor set, which can maximize the difficulty of multiple-choice questions, rather than picking prediction results with the highest probability but with similar semantic. 

Based on this view, we propose to incorporate a multi-choice reading comprehension (MRC) model for ranking/selecting distractor sets. First, let $\mathbb{M}_{\texttt{MRC}}$ be a MRC model. Note that $\mathbb{M}_{\texttt{MRC}}$ takes a context passage $P$, a question $Q$, and a set of options (including an answer phrase $A$ and distractors $D_1, D_2, ..., D_n$) as input and outputs [$p_A, p_{D_1}, ...,p_{D_n}$] as the answer probabilities of the options with respect to the context passage $P$ and the question $Q$. $\mathbb{M}_{\texttt{MRC}}$ is trained by maximizing the answer probability $p_A$ while minimizing the probabilities [$p_{D_1}, ...,p_{D_n}$]. 

With $\mathbb{M}_{\texttt{MRC}}$, our idea is as follows. First, let $\mathbb{DG}_{\texttt{BDG}}$ be the BDG model for distractor generation. Also, let $\hat{D}=\{\hat{d}_1, \hat{d}_2, ..., \hat{d}_n\}$ be the set of generated distractors by the BDG model. In a common MCQ setting, there are four options (one answer $A$ and three distractors $d_i, d_j, d_k$) for each question. Our idea is to enumerate all possible triples from $\{\hat{d}_1, \hat{d}_2, ..., \hat{d}_n\}$. That is, we have a triple set 
\[
  \{ (d_i, d_j, d_k)| i\neq j\neq k, d_i, d_j, d_k \in \hat{D} \}
\]

For a given passage $P$, question $Q$, and answer $A$, the goal is to find a triple ($d_i, d_j, d_k$) to form an option set $O$ (i.e., \{$d_i, d_j, d_k$, $A$\} ) that maximizes the following entropy function.

\begin{equation}\label{eq:entropy}
    \underset{}{\text{maximize}}-\sum_{\forall o_i\in O}p_{o_i}log_2p_{o_i}
\end{equation}



\subsection{Model Ensemble}\label{sec:model-ensemble}
The idea of selecting distractors by entropy maximization can be further generalized by employing multiple DG models. For having multiple DG models, our idea is to leverage the variants of the \BDGname model (i.e., models with/without answer negative regularization or with/without P-MLM multi-task training). Let $\hat{D}, \hat{D}_{_{ \neg A.}}$, and $\hat{D}_{_{\neg P.}}$ be the full DG model, the DG model without answer negative regularization, and the DG model without P-MLM multi-task training.
With the models, our goal then can be to enumerate all  possible triples from $\{\hat{d}_1, \hat{d}_2, ..., \hat{d}_n\}$. That is, we have a triple set as follows.
\[
  \{ (d_i, d_j, d_k)| d_i \in \hat{D}, d_j \in \hat{D}_{_{ \neg A.}}, d_k \in \hat{D}_{_{\neg P.}} \}
\]

With the triple set, the options set that maximizes Eq. (\ref{eq:entropy}) is selected as final distractors.



% \noindent\textbf{RACE}
% Token level (e.g., bleu score, rouge-l) performance evaluation fail to truly reflect the quality of generated distractors. We propose to evaluate the DG quality by RACE reading comprehension task \cite{lai2017large} (Race is a large-scale reading comprehension dataset with more than 28,000 passages and nearly 100,000 questions. In the dataset, all questions contain four candidate options with only one correct option. Our idea is that a poorly generated result will reduce the difficulty of the multiple-choice task. We expect that this effect will be reflected in the phenomenon that the accuracy of a multiple choice model is improved. Thus, we propose to incorporate a RACE model to test the accuracy of a multiple choice quiz that uses the distractors generated by our model. Specifically, given $C$, $Q$, and $A$, we generate three distractors $D_1$, $D_2$, and $D_3$, and then turn the multiple choice question to the implemented RACE model. We expect that the randomly generated results will significantly increase the accuracy of the model. Therefore, we hope to reflect the quality of the results through such a way of comparison.

% In the experiment, we implement a RACE model based on  RoBERTa fine-tuned by OpenAI \cite{solaiman2019release} to realize our idea. We use the accuracy of the model as a metric. The higher the accuracy, the worse the generation quality. In Table \ref{tab:acc}, we show the results. 

% \begin{table}[ht]\centering
% \begin{tabular}{|l|r|}
% \hline
%  & \multicolumn{1}{l|}{Accuracy} \\ \hline
% Random Generator & 87.79\% \\ \hline
% Golden Distractor & 78.39\% \\ \hline
% BERT-DG & 73.39\% \\ \hline
% \end{tabular}
% \caption{Accuracy Comparison on RACE }
% \label{tab:acc}
% \end{table}





% \subsection{Generating Multiple Distractors}
% In addition to a single distractor generation, we also target at generating multiple distractors. To increase the quality of the distractors (the quality is defined in terms of increasing the difficulty of multiple-choice questions), we also employ the unlikelihood loss idea as we introduced in Eq. (\ref{eq:SLUL}) but to regulate $D_2$ use words different from the words of $A$ and $D_1$.
